LeakyPick: IoT Audio Spy Detector

Manufacturers of smart home Internet of Things (IoT) devices are increasingly adding voice assistant and audio monitoring features to a wide range of devices including smart speakers, televisions, thermostats, security systems, and doorbells. Consequently, many of these devices are equipped with microphones, raising significant privacy concerns: users may not always be aware of when audio recordings are sent to the cloud, or who may gain access to the recordings. In this paper, we present the LeakyPick architecture that enables the detection of the smart home devices that stream recorded audio to the Internet without the user's consent. Our proof-of-concept is a LeakyPick device that is placed in a user's smart home and periodically "probes" other devices in its environment and monitors the subsequent network traffic for statistical patterns that indicate audio transmission. Our prototype is built on a Raspberry Pi for less than USD40 and has a measurement accuracy of 94% in detecting audio transmissions for a collection of 8 devices with voice assistant capabilities. Furthermore, we used LeakyPick to identify 89 words that an Amazon Echo Dot misinterprets as its wake-word, resulting in unexpected audio transmission. LeakyPick provides a cost effective approach for regular consumers to monitor their homes for unexpected audio transmissions to the cloud.

==> hiddenwakewords.tex <==
%!TeX root=LeakyPick.tex


==> motivation.tex <==
%!TeX root=LeakyPick.tex

Recent reports about big Internet companies like Amazon~\cite{Bloomberg2019}, Google~\cite{Google2019, VRTNews2019}, Apple~\cite{TheGuardian2019}, Microsoft~\cite{Motherboard2019} and Facebook~\cite{Bloomberg2019-2} that offer voice-activated and voice-controlled services have revealed that employees and subcontractors of these companies are tasked with listening to and interpreting audio recordings captured by respective voice assistant devices in connection to potentially misinterpreted voice commands, or, commands that were not intended to be addressed to the assistant in question. Such recordings are made, e.g., when an assistant device misunderstands a part of a spoken sentence as its ``wake-word'', i.e., a word or a phrase that is intended to be used by the user to activate the assistant to listen to subsequent voice commands. However, as unintentional audio recordings made by such devices may reveal very sensitive information about persons in the vicinity, they pose a significant privacy threat, especially as users may not be aware of such recordings being made. 

%This brings us to the second motivation of this paper, finding out on which words voice assistants such as Alexa, Google Assistant, Siri or Cortana are reacting in addition to the specified ones.
A similar privacy threat may also arise due to potential malicious or semi-honest IoT device manufacturers, who integrate voice or audio sensing capabilities to IoT devices manufactured by them without openly documenting this in the product documentation of the device. For example, recently it was revealed that Google failed to disclose the presence of a microphone in one of their Google Nest products~\cite{BusinessInsider2019}. For such devices, there is no apparent way for the users of such devices to be aware of the fact that any audio recordings of them may even be made.

To encounter threats related to audio recordings made without the knowledge or approval of users we therefore develop an approach based on an audio-probing device that is able to detect devices in a user's home that react to voice-based audio inputs and transmit data outside the user's home network. The detection approach is based on the assumption that IoT devices reacting to audio commands typically send out data to their respective back-end services immediately as the interpretation and consequent actions in response to the inputs are typically performed by voice-recognition algorithms and services running in the cloud-based back-end of the respective device or service vendor. 
Our approach is based on active audio probing aiming at identifying possible devices reacting to audio by observing the network communications of devices in the user's home network subsequent to the probing event.
% injecting potential wake-words into the audio context and monitoring the resulting network communications of devices in the user's network, we seek to identify such devices that with high likelihood are programmed to react to audio and transmit audio recording to external entities outside the user's network.

During the course of our investigation, we discovered that also other words than the designated wake words can activate the voice-activated functionalities of voice-controlled devices.
As such it is not surprising that background noise such as dialogues between persons, a TV or radio broadcast or even specific household background sounds may be mistaken by voice assistants as their wake word. However, how widespread such unintended voice activations with voice assistant devices are has---to the best of our knowledge---not been investigated systematically so far. In order to quantify the extent of this problem, we therefore perform systematic measurements with which we seek to find out how sensitive voice assistant systems are in practice to misinterpret various inputs of normal human language as their wake word. Somewhat surprisingly, as our evaluation in Sect.~\ref{sect:evaluation} shows, it turns out that voice assistants not only react to their designated wake words and utterances bearing similarity with the wake word, but also to utterances that seemingly do not have any apparent similarity with any of the declared wake words. This result suggests that unintended voice recordings performed by IoT voice assistant devices may pose a significant threat to the personal privacy of users employing such devices in their homes.

%Sometimes it is unknown if a device listens to audio and is sending data over Wi-Fi to the outside world or if it is known that a device can send audio it may be unknown exactly when a device is listening and sending.




